Good News Is Not a Sufficient Condition for Motivated Reasoning

People often receive good news that makes them feel better about the world around them, or bad news that makes them feel worse about it. This paper studies how the valence of news affects belief updating, absent functional and ego-relevant factors. Using experiments with over 1,500 participants and 5,600 observations, I test whether people engage in motivated reasoning to overly trust good news versus bad news on valence-relevant issues like cancer survival rates, others' happiness, and infant mortality. The estimate for motivated reasoning towards good news is a precisely-estimated null. Modest effects, of one-third the size of motivated reasoning in politics and performance, can be ruled out. Complementary survey evidence shows that most people expect good news to increase happiness, but to not systematically lead to motivated reasoning. These results suggest that belief-based utility is not sufficient in leading people to distort belief updating in order to favor those beliefs.

==> change_guess_positivity.tex <==
\begin{tabular}{l*{4}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
\hline
Good News           &   -0.003&    0.005&    0.025&    0.021\\
                    &  (0.016)&  (0.017)&  (0.031)&  (0.024)\\
Bad News            &         &         &    0.015&         \\
\hspace{35mm}       &         &         &  (0.031)&         \\
Pro-Party News      &         &         &         &    0.043\\
                    &         &         &         &  (0.024)\\
Question FE         &      Yes&      Yes&       No&      Yes\\
Round FE            &      Yes&      Yes&      Yes&      Yes\\
Subject FE          &       No&      Yes&      Yes&      Yes\\
Subject controls    &      Yes&       No&       No&       No\\
Neutral News        &       No&       No&      Yes&       No\\
\hline
Observations        &     5692&     5464&     5972&     2706\\
Subjects            &     1521&     1293&     1293&      658\\
Mean                &    0.635&    0.635&    0.635&    0.661\\
\hline\hline
\multicolumn{5}{l}{\footnotesize Standard errors in parentheses}\\
\end{tabular}


==> change_guess_positivity_failedcheck.tex <==
\begin{tabular}{l*{4}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
\hline
Good News           &    0.030&    0.032&    0.029&    0.060\\
                    &  (0.015)&  (0.016)&  (0.026)&  (0.022)\\
Bad News            &         &         &   -0.007&         \\
\hspace{35mm}       &         &         &  (0.026)&         \\
Pro-Party News      &         &         &         &   -0.002\\
                    &         &         &         &  (0.023)\\
Question FE         &      Yes&      Yes&       No&      Yes\\
Round FE            &      Yes&      Yes&      Yes&      Yes\\
Subject FE          &       No&      Yes&      Yes&      Yes\\
Subject controls    &      Yes&       No&       No&       No\\
Neutral News        &       No&       No&      Yes&       No\\
\hline
Observations        &     8687&     8373&     9273&     3741\\
Subjects            &     2305&     1991&     1991&      912\\
Mean                &    0.522&    0.522&    0.522&    0.553\\
\hline\hline
\multicolumn{5}{l}{\footnotesize Standard errors in parentheses}\\
\end{tabular}


==> moreas_and_guess_positivity_failed.tex <==
\begin{tabular}{l*{8}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}&\multicolumn{1}{c}{(8)}\\
                     &\multicolumn{4}{c}{Dep Var: News Assessments}&\multicolumn{4}{c}{Dep Var: Changing Guesses}\\
\hline
Good News           &   -0.002&   -0.008&   -0.000&   -0.002&    0.030&    0.032&    0.060&    0.060\\
                    &  (0.005)&  (0.005)&  (0.007)&  (0.007)&  (0.015)&  (0.016)&  (0.022)&  (0.022)\\
Pro-Party News      &         &         &    0.041&    0.042&         &         &   -0.002&   -0.002\\
                    &         &         &  (0.008)&  (0.008)&         &         &  (0.023)&  (0.023)\\
Question FE         &      Yes&      Yes&      Yes&      Yes&      Yes&      Yes&      Yes&      Yes\\
Round FE            &      Yes&      Yes&      Yes&      Yes&      Yes&      Yes&      Yes&      Yes\\
Subject FE          &       No&      Yes&       No&      Yes&       No&      Yes&      Yes&      Yes\\
Participant controls &      Yes&       No&      Yes&       No&      Yes&       No&      Yes&       No\\
\hline
Observations        &     8687&     8373&     4102&     3741&     8687&     8373&     3741&     3741\\
Participants        &     2305&     1991&     1273&      912&     2305&     1991&      912&      912\\
Mean                &    0.557&    0.557&    0.557&    0.557&    0.522&    0.522&    0.553&    0.553\\
\hline\hline
\multicolumn{9}{l}{\footnotesize Standard errors in parentheses}\\
\end{tabular}


==> moreas_positivity.tex <==
\begin{tabular}{l*{4}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
\hline
Good News           &   -0.002&   -0.002&    0.011&    0.002\\
                    &  (0.006)&  (0.007)&  (0.013)&  (0.009)\\
Bad News            &         &         &    0.012&         \\
\hspace{35mm}       &         &         &  (0.013)&         \\
Pro-Party News      &         &         &         &    0.054\\
                    &         &         &         &  (0.010)\\
Question FE         &      Yes&      Yes&       No&      Yes\\
Round FE            &      Yes&      Yes&      Yes&      Yes\\
Subject FE          &       No&      Yes&      Yes&      Yes\\
Subject controls    &      Yes&       No&       No&       No\\
Neutral News        &       No&       No&      Yes&       No\\
\hline
Observations        &     5692&     5464&     5972&     2706\\
Subjects            &     1521&     1293&     1293&      658\\
Mean                &    0.576&    0.576&    0.576&    0.575\\
\hline\hline
\multicolumn{5}{l}{\footnotesize Standard errors in parentheses}\\
\end{tabular}


==> moreas_positivity_failedcheck.tex <==
\begin{tabular}{l*{4}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
\hline
Good News           &   -0.002&   -0.008&    0.007&   -0.002\\
                    &  (0.005)&  (0.005)&  (0.009)&  (0.007)\\
Bad News            &         &         &    0.015&         \\
\hspace{35mm}       &         &         &  (0.009)&         \\
Pro-Party News      &         &         &         &    0.042\\
                    &         &         &         &  (0.008)\\
Question FE         &      Yes&      Yes&       No&      Yes\\
Round FE            &      Yes&      Yes&      Yes&      Yes\\
Subject FE          &       No&      Yes&      Yes&      Yes\\
Subject controls    &      Yes&       No&       No&       No\\
Neutral News        &       No&       No&      Yes&       No\\
\hline
Observations        &     8687&     8373&     9273&     3741\\
Subjects            &     2305&     1991&     1991&      912\\
Mean                &    0.557&    0.557&    0.557&    0.557\\
\hline\hline
\multicolumn{5}{l}{\footnotesize Standard errors in parentheses}\\
\end{tabular}

